FedABC: Targeting Fair Competition in Personalized Federated Learning

Federated learning aims to collaboratively train models without accessing their client's local private data. The data may be Non-IID for different clients and thus resulting in poor performance. Recently, personalized federated learning (PFL) has achieved great success in handling Non-IID data by enforcing regularization in local optimization or improving the model aggregation scheme on the server. However, most of the PFL approaches do not take into account the unfair competition issue caused by the imbalanced data distribution and lack of positive samples for some classes in each client. To address this issue, we propose a novel and generic PFL framework termed Federated Averaging via Binary Classification, dubbed FedABC. In particular, we adopt the ``one-vs-all'' training strategy in each client to alleviate the unfair competition between classes by constructing a personalized binary classification problem for each class. This may aggravate the class imbalance challenge and thus a novel personalized binary classification loss that incorporates both the under-sampling and hard sample mining strategies is designed. Extensive experiments are conducted on two popular datasets under different settings, and the results demonstrate that our FedABC can significantly outperform the existing counterparts.

==> Fig_Non_iid/test.tex <==
\begin{equation}
\begin{split}
{E}\left[\mathcal{L}^{\textit{BCE}}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};{\theta_{i}} \right)\right]:=&\frac{1}{|\mathcal{S}^{i}|} \left(\sum_{j}^{C_{i}^{p}}{L}^{p}_\textit{BCE}(\mathcal{S}^{i};{\theta}_{i})+\sum_{j}^{C_{i}^{n}} L_{\textit{BCE}}^{n}(\mathcal{S}^{i};{\theta}_{i}) \right).
\end{split}
\end{equation}

==> text/abstract-V1.tex <==

\begin{abstract}
Federated learning aims to collaboratively train models on the network edge without accessing their client's private data, which faces the problem of learning with Non-IID data and thus resulting
in poor performance. To cope with it, the huge success of personalized federated learning have achieved by enforcing regularization in local optimization or improving the model aggregation scheme at the server. However, most previous works do not take into account the issue that existing different situations between classes amongst clients, which induces unfair competition and sub-optimal performance for the significant problem of imbalanced
data distributions and the lack of positive samples. To remedy these drawbacks, we propose a novel and generic federated binary classification training method termed Personalized Federated Averaging Learning Via Adopting Binary Classification methods, dubbed FedBC, to bridge this gap in personalized federated learning. Our method integrates the “one-vs-all” framework to reduce the impact and unfair competition between classes and thus be more focused on personalized classes. Specifically, our method employs the under-sampling and hard sample mining strategy to alleviate the imbalance problem and the lack of positive samples. Extensive experiments on multiple popular datasets(MNIST, CIFAR-10) are conducted under
different heterogeneous settings, which demonstrates that our FedBC can significantly outperform existing counterparts.

\end{abstract}

==> text/abstract.tex <==

\begin{abstract}
Federated learning aims to collaboratively train models without accessing their client's local private data.  The data may be Non-IID for different clients and thus resulting in poor performance. Recently, personalized federated learning (PFL) has achieved great success in handling Non-IID data by enforcing regularization in local optimization or improving the model aggregation scheme on the server. However, most of the PFL approaches do not take into account the unfair competition issue caused by the imbalanced data distribution and lack of positive samples for some classes in each client. To address this issue, we propose a novel and generic PFL framework termed Federated Averaging via Binary Classification, dubbed FedABC. In particular, we adopt the ``one-vs-all'' training strategy in each client to alleviate the unfair competition between classes by constructing a personalized binary classification problem for each class. This may aggravate the class imbalance challenge and thus a novel personalized binary classification loss that incorporates both the under-sampling and hard sample mining strategies is designed. Extensive experiments are conducted on two popular datasets under different settings, and the results demonstrate that our FedABC can significantly outperform the existing counterparts.
\end{abstract}



==> text/conclusion-V1.tex <==
\section{Conclusion}
In this paper, we investigate the Non-iidd problem in the federated learning setting, where the data distribution among clients is imbalanced and some classes even have no positive samples, and propose a novel algorithm FedABC to address this issue. Concretely, our method treats each class as a binary classification problem and train a binary classifier for every classes. Adopting this training method can liberate classes from unfair competition caused by imbalanced data distribution in some degree. This training method may aggravate the class imbalance problem and thus the under-sampling and hard sample mining are further utilized. Extensive experiments
are conducted on multiple popular datasets show that our FedABC can significantly improve the PFL performance and thus alleviate the Non-iid problem.



==> text/conclusion.tex <==
\section{Conclusion}
In this paper, we investigate some extraordinary Non-IID situations in federated learning, where the data distributions among clients are imbalanced and some classes even have no positive samples. These issues are alleviated by constructing a binary classification problem for each category instead of adopting the popular Softmax function. This training strategy may aggravate the class imbalance problem and thus a novel loss function that incorporates the under-sampling and hard sample mining are further designed. Extensive experiments are conducted on two popular datasets, and the results show that our FedABC can significantly improve the PFL performance in diverse heterogeneity settings. In the future, we intend to integrate with the communication strategies to further improve the performance and conduct experiments on more large-scale datasets.



==> text/experiments.tex <==
\section{Experiments}

\subsection{Setup}

\paragraph{Datasets.}We use the MNIST~\cite{1998Gradient} and CIFAR-10~\cite{2009Learning} as benchmark. To simulate the heterogeneous federated learning scenario, we follow previous works ~\cite{yurochkin2019bayesian,wang2020federated} that utilizes the Dirichlet distribution
$Dir(\alpha)$ to partition the training dataset and generate the corresponding test data for each client following the same distribution, in which a smaller $\alpha$ indicates the higher data heterogeneity. In our experiment, the number of total users is 20. We follow the visualization method in previous work~\cite{zhu2021data} to visualize the statistical heterogeneity of clients, the results are shown in Figure \ref{fig:label-heterogeneity}. 
\paragraph{Model.}For MNIST, we use the fully connected network, the network contains 3 FC layers, the FC layers are with 260, 200 hidden size and 10 neurons for 10 classes as output. Since we adopt the binary training strategy, the binary activation function \textbf{sigmoid} is applied and maps the output into the interval $[0,1]$. Instead, we normally apply softmax activation for the compared methods. For CIFAR-10, we use the ConvNet~\cite{lecun1998gradient}, it contains 2 Conv layers and 3 FC layers. The Conv layers have 64 and 64 channels, respectively. The FC layers are with 120, 64 hidden size and 10 neurons as output. Same as the fully connected network used on MNIST, the the binary activation function sigmoid is applied. 
\paragraph{Configuration.}Our method has four hyper-parameters: $m^{p}$,${m^{n}}$,$m^{nn}$ and $\alpha$. These parameters amongst different clients can be varied according to the local imbalanced situation, but we make them equal in the simplest way. For CIFAR-10, we set them as $0.85$, $0.2$, $0.3$ and $2$, respectively. For MNIST, we set them as $0.75$, $0.25$, $0.3$ and $2$, respectively. Throughout
the experiments, we use the SGD optimizer with weight decay $1e-5$ and a $0.9$ momentum. For MNIST, the learning rate is $0.01$. For CIFAR-10, the learning rate is $0.1$. we train every method for $100$ rounds and $200$ rounds in the MNIST and CIFAR-10 experiments, respectively. For federated framework setting, the participation rate of clients is set as $0.5$, it means that random $10$ clients are activated in each communication round. The local training epoch is set as $5$ for all the experiments.
\paragraph{Compared methods.}We follow the observation~\cite{chen2021bridging} that if we adopt personalized models in generic FL algorithms, they outperform nearly all the existing P-FL algorithms. so we select some challenging generic FL algorithms including FedAvg~\cite{mcmahan2017communication}, FedProx~\cite{li2020federated}, Scaffold~\cite{karimireddy2020scaffold} and evaluate their personalized model. For PFL methods, LG\_FedAvg~\cite{liang2020think}, FedPer~\cite{2019Federated}, FedRep~\cite{collins2021exploiting} and FedRod~\cite{chen2021bridging}
are selected. In particular, FedRod has double classifier layers to perform on global model and personalized model, respectively. In our experiments, FedRod adopts the linear strategy that only G-Head is aggregated at the server.   


\begin{figure*}[!t]  
    \begin{center}
       
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Mnist_0.1.pdf}}
        \subcaption{\small MNIST$(\alpha=0.1)$}
        \end{subfigure} 
        % 
        \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Mnist_0.3.pdf}}
        \subcaption{\small MNIST$(\alpha=0.3)$}
        \end{subfigure} 
        % 
         \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Mnist_0.5.pdf}}
        \subcaption{\small MNIST$(\alpha=0.5)$}
        \end{subfigure} 
        % 
          \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Mnist_1.0.pdf}}
        \subcaption{\small MNIST$(\alpha=1.0)$}
        \end{subfigure} 
        %  
        
        
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Cifar10_0.1.pdf}}
        \subcaption{\small CIFAR-10$(\alpha=0.1)$}
        \end{subfigure} 
        % 
         \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Cifar10_0.3.pdf}}
        \subcaption{\small CIFAR-10$(\alpha=0.3)$}
        \end{subfigure} 
        % 
         \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Cifar10_0.5.pdf}}
        \subcaption{\small CIFAR-10$(\alpha=0.5)$}
        \end{subfigure} 
        % 
         \hspace{0.1in}
        \begin{subfigure}[b]{0.23\textwidth}
            \centerline{\includegraphics[width=1.2\columnwidth]{Fig_Non_iid/Cifar10_1.0.pdf}}
        \subcaption{\small CIFAR-10$(\alpha=1.0)$}
        \end{subfigure} 
        %  
 
    \caption{Visualization of statistical heterogeneity among clients, where the $x$-axis indicates user IDs, the $y$-axis indicates class labels, and the size of scattered points indicates the number of training samples.}\label{fig:label-heterogeneity}
    \end{center}
\end{figure*} 

\begin{table*}[!t]

%h：hear，t：top，b：bottom，p：page，下一页。
\caption{ P-FL accuracy(\%) on MNIST and CIFAR-10 with different degrees of heterogeneity (0.1, 0.3, 0.5, 1.0). The underline highlight the best baseline approach.}
\centering
\label{tab1}
 \resizebox{\textwidth}{!}{
 \begin{tabular}{c|c|cccc|ccccc}    
         \toprule       
         %最上面的横线
        {Dataset}& {Non-iid}&{Local only}&{FedAvg}&{FedProx}&{Scaffold}&{LG\_FedAvg}& {FedPer}&{FedRep}&{FedRod}&{FedABC}\\ 
        \midrule
        \multirow{4}{*}{MNIST}&{Dir(0.1)}&{97.1}&{99.1}&{98.4}&{99.3}&{99.2}&{99.1}&{98.9}&{
        \uline{99.3}}&\textbf{99.3}\\
       % \cmidrule{2-11}
         \multirow{4}{*}{}&{Dir(0.3)}    &{93.3}&{98.3}&{97.1}&{98.6}&{98.2}&{98.2}&{97.8}& \uline{98.7}&\textbf{98.7}\\
         %\cmidrule{2-11}
        
        \multirow{4}{*}{}&{Dir(0.5)}     &{92.1}&{98.1}&{96.9}&{98.5}&{98.1}&{98.0}&{97.6}& \uline{98.6}&{98.5}\\
        %\cmidrule{2-11}
        \multirow{4}{*}{}&{Dir(1.0)}     &{90.6}&{98.0}&{96.9}&{98.4}&{98.1}&{98.1}&{97.4}& \uline{98.5}&\textbf{98.7}\\
        
        %CIFAR-10
        \midrule
        \multirow{4}{*}{CIFAR-10}&{Dir(0.1)}&{86.0}&{91.0}&{91.1}& \uline{91.2}&{88.7}&{90.2}&{90.4}&{90.5}&{91.0}\\
        %\cmidrule{2-11}
         \multirow{4}{*}{}&{Dir(0.3)}      &{72.4}&{82.1}&{82.2}&{81.9}&{76.6}&{81.2}&{81.4}& \uline{82.2}&\textbf{83.3}\\
         %\cmidrule{2-11}
        
        \multirow{4}{*}{}&{Dir(0.5)}       &{67.8}&{79.8}&{79.3}&{79.5}&{72.8}&{78.8}&{79.1}& \uline{79.8}&\textbf{81.1}\\
        %\cmidrule{2-11}
        \multirow{4}{*}{}&{Dir(1.0)}       &{83.7}&{74.1}&{73.8}&{74.0}&{63.7}&{72.5}&{73.4}&\uline{74.1}&\textbf{76.1}\\
       \bottomrule
       
    %     {Non-IID}&\multicolumn{3}{c|}{Dir(0.1)}& \multicolumn{3}{c}{Dir(0.3)}& \multicolumn{3}{c|}{Dir(0.5)}& \multicolumn{3}{c|}{Dir(1.0)}& \multicolumn{3}{c|}{Dir(0.1)}& \multicolumn{3}{c|}{Dir(0.3)}& \multicolumn{3}{c|}{Dir(0.5)}&  \multicolumn{3}{c}{Dir(1.0)}  \\
     
    \end{tabular}}
\end{table*}

\subsection{Evaluation criteria}
\paragraph{Evaluation of personalized model.}To simulate the Non-iid setting in FL, each client has local train set and the corresponding test set with the same Dirichlet distribution. For evaluation on PFL, we use the Non-iid test set and the formulation can be given by the following:
\begin{equation}
\small
\textbf{PFL-accuracy: } T_{\text{PFL}}=\frac{\sum_{i} {I(y_{j}=\hat{y_{j}};D_{\footnotesize \text{ Non\_iid\_test}}^{i};\boldsymbol{\theta}^{i})}}{\sum_{i}|D^{i}_{\footnotesize \text{ Non\_iid\_test}}|}
\label{eva-PFL}
\end{equation}
where $I(\cdot)$ is an indicator function ($I(E)=1$ if event $E$ is true, and $0$ otherwise). The PFL test accuracy is obtained from the the sum of all the local true predictions number divided by the sum of the number of all test set. It is emphasized that the local testing process utilizes the personalized model instead of the global model.
\paragraph{Evaluation of Client Drift.}In our work, we also propose an evaluation method to quantity the degree of client drift. Due to the varied data distributions, the local training performs with biases towards the local classes and easily forget other information, including other classes feature or different feature of the same class. To quantify the degree of client drift, we can test the personalized model on the iid test set and treat the resulted accuracy as the metric of client drift. Employing this evaluation method, the low accuracy indicates that a high degree of drift occurrence while the great accuracy indicates that local training does not completely forget other knowledge. This formulation can be given by the following:
\begin{equation}
\small
\textbf{PFL-accuracy: } T_{\text{PFL}}=\frac{\sum_{i} {I(y_{j}=\hat{y_{j}};D^{i}_{\footnotesize \textbf{iid\_test}};\boldsymbol{\theta}^{i})}}{\sum_{i}|D^{i}_{\footnotesize \textbf{iid\_test}}|}
\label{eva-PFL}
\end{equation}
\subsection{Results and analysis}
We present the results in the Tables \ref{tab1} \&\ref{tab2}, underline and fonts highlight the best baseline/our approach. From the experiment results, we observe that: 1)the advanced local training of generic FL can achieve good accuracy and even outperforms other PFL algorithms, especially in the huge heterogeneity setting(i.e.,0.1). The reason behind this is that the data distribution of test data is same with the training data. In this case, there are very few classes amongst clients, so that the low accuracy of the minority classes can not impact on the final accuracy and thus achieve unexpected results. To understand better, we assume that each clients only access to a single class, and the PFL accuracy in this setting will be amazing $100\%$; 2) the accuracy of PFL decrease with the level of heterogeneity, the local training is hard to cater for all class due to the lacking feature and more class information; 3) The FedRod achieves the most sota compared with other baselines, especially in the MNIST experiments. FedRod has double classifiers for global paradigm and personalized paradigm and can be more robust. 4) Regard to the PFL accuacy, FedABC achieves promising performance and outperforms other baselines. 4) Regard to the client drift, Scaffold uses control variates to correct for the ‘client-drift’ in its local updates and thus achieve the best performance. Our FedABC also achieve good performance compared with other methods.

FedABC achieves the highest P-FL accuracy in most cases and benefit from its binary training method. In the MNIST experiment, FedABC achieve the performance Slightly better than the SOTA method FedRod. Regards to the CIFAR-10 experiments, our FedABC significantly outperforms the competitive counterpart. Besides, in the experiment of client drift, FedABC can also combat catastrophic forgetting to a certain extent. The reason behind the promising results is that FedABC adopts the binary training method that can address unfair competition between classes and significantly improve the local training process.
\begin{table*}[!t]

%h：hear，t：top，b：bottom，p：page，下一页。
\caption{Table illustrating drift degree of different methods, The Quantification of clients drift is achieved from the personalized model accuracy tested on iid test set. Lower values mean a greater degree of drift. The The underline highlight the best baseline approach.}
\centering
\label{tab2}
 \resizebox{\textwidth}{!}{
 \begin{tabular}{c|c|cccc|ccccc}    
         \toprule       
         %最上面的横线
        {Dataset}& {Non-iid}&{Local only}&{FedAvg}&{FedProx}&{Scaffold}&{LG\_FedAvg}& {FedPer}&{FedRep}&{FedRod}&{FedABC}\\ 
        \midrule
        \multirow{4}{*}{MNIST}&{Dir(0.1)}&{29.2}&{43.7}&{39.4}&\uline{76.8}&{43.9}&{43.7}&{42.9}&{{66.9}}&\textbf{76.5}\\
       % \cmidrule{2-11}
         \multirow{4}{*}{}&{Dir(0.3)}  &{44.2}&{68.2}&{62.2}&\uline{90.2}&{68.1}&{68.2}&{66.3}&{85.4}&\textbf{91.1}\\
        %\cmidrule{2-11}
        
        \multirow{4}{*}{}&{Dir(0.5)}     &{58.0}&{78.7}&{74.0}&\uline{94.0}&{78.7}&{78.8}&{77.1}&{90.8}&\textbf{95.1}\\
        %\cmidrule{2-11}
        \multirow{4}{*}{}&{Dir(1.0)}     &{69.5}&{87.6}&{84.9}&\uline{97.0}&{87.6}&{87.6}&{86.4}&{95.3}&\textbf{97.2}\\
        
        %CIFAR-10
        \midrule
        \multirow{4}{*}{CIFAR-10}&{Dir(0.1)}&{16.7}&{37.0}&{37.8}&\uline{39.6}&{20.6}&{38.6}&{23.5}&{31.5}&\textbf{34.5}\\
        %\cmidrule{2-11}
         \multirow{4}{*}{}&{Dir(0.3)}      &{23.3}&{56.4}&{56.3}&\uline{56.1}&{32.1}&{42.0}&{41.6}&{51.4}&\textbf{54.7}\\
         %\cmidrule{2-11}
        
        \multirow{4}{*}{}&{Dir(0.5)}       &{25.6}&{60.0}&{59.9}&\uline{60.0}&{35.4}&{47.0}&{46.5}&{55.5}&\textbf{59.0}\\
        %\cmidrule{2-11}
        \multirow{4}{*}{}&{Dir(1.0)}       &{14.4}&{64.8}&{64.2}&\uline{65.2}&{39.7}&{52.7}&{53.8}&{61.5}&\textbf{64.0}\\
       \bottomrule
    \end{tabular}}
\label{client_drift}
\end{table*}

\paragraph{Ablation Study}
\begin{figure}[!t]
    \begin{center}
    \includegraphics[width=0.8\columnwidth]{ablation_study.pdf}
    \end{center}
    \caption{The blue column represents our FedABC integrating with under-sampling and hard sample mining strategy. The compared method FedABC$\_$wi who does not adopt our imbalanced training techniques is represented by the orange column.}
    \label{Ablation study}
\end{figure}
we study the necessity of component for solving imbalanced problem in our binary classification. we conduct the ablation experiments on CIFAR-10. Same as the previous configuration, we train 200 epochs for the compared FedABC\_wi without adopting our imbalanced training technique(under-sampling and hard sample mining), the experiments results are shown in Figure \ref{Ablation study}. From the Figure, we can find that: 1) Adopting our imbalanced training technique can improve the performance. The P-FL accuracy improvement is $0.3\%$, $1.0\%$, $1.4\%$, $1.6\%$ for the heterogeneity setting $0.1$, $0.3$, $0.5$, $1.0$, respectively. The positive samples and negative samples sometimes is serious imbalanced in our binary classification for each class and the efficient imbalanced training technique can alleviate it and thus generate improvement; 2) The accuracy improvement is decrease with the degree of heterogeneity. In huge heterogeneity setting(e.g. Dir(0.1)), the improvement is slight and Significantly efficient for the other setting. The reason is that re-balancing data distribution may generate the trade off between the PFL accuracy and the imbalanced problem. Since the data distribution of test set is same with the train set, the excessive re-balancing may inevitably hurts the local model personalized performance. However, training with serious imbalanced problem can also impact the classify decision on minority classes, especially in our binary training strategy.



==> text/introduction-V1.tex <==
\section{Introduction}
Federated learning~\cite{mcmahan2017communication}(FL) is an emerging machine learning  paradigm that trains an algorithm across multiple decentralized clients (such as edge devices) or servers without exchanging local data samples. In the real word, large-scale data are becoming increasingly popular with the advent of the big data era but come with the risk of data privacy. Federated learning aims at addressing this issue by providing the platform in which clients update models on their devices using private data and the server periodically averages these models for multiple communication rounds. Such decentralized learning has shown its potential to facilitate real-world applications, including healthcare\cite{xu2021federated}, user verification\cite{hosseini2021federated} and the Internet of Things (IoT)\cite{zheng2022applications}.

A notorious trap in federated learning is training with non-independent and
identically distributed (non-i.i.d.) data\cite{hsieh2020non}. Due to diverse client's data distributions, the single global model obtained by simply averaging is hard to cater for all heterogeneous clients. Besides, clients update the global model on their local dataset, making local model misaligned and leading to weight divergence\cite{zhao2018federated}. These problems have been found to result in unstable and slow convergence \cite{li2020federated}and even extremely poor performance \cite{li2021federated}.
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1\columnwidth]{AAAI_figure_1.pdf}
    \end{center}
    \caption{}
    \label{fig:1}
\end{figure}

To deal with heterogeneity in FL, numerous of works have been exploit promising solutions, among which these methods\cite{li2020federated,karimireddy2020scaffold,acar2021federated} constrain the direction of local model update
to align the local and global optimization objectives. Besides, personalized Federated Learning(PFL)(\cite{smith2017federated} addresses this challenge by jointly learning a personalized model for each client. For instance, \cite{collins2021exploiting,liang2020think,sun2021partialfed} exploit flexible parameter sharing strategies that only transmitting partial model parameters. \cite{t2020personalized,hanzely2020lower,li2021ditto} regularized local models with a learnable global model.

However, all these methods merely conduct an extra regularization or improving the aggregation strategy, which ignore extraordinary situations of data distribution(see \ref{fig:1}) existing in FL clients. The situations can be divided into two categories: 1) imbalanced class distribution\cite{he2009learning}, some classes have more or less samples than others; 2) lacking positive samples, some classes only have negative samples without positive samples, the probability of occurrence increases with the degree of heterogeneity; Along with these facts, we further dig deeper into the process of client optimization. Ubiquitous Softmax (cross-entropy)\cite{jang2016categorical} normalization enforces all the class logits summed to one, inducing competition among different classes and thus increasing the confidence of one class will necessarily decrease the confidence
of some other classes. In our case, since the imbalanced training samples and unfair competition, these two situation can easily lead to over-confident predictions\cite{guo2017calibration} for dominated classes, sub-optimal performance for minority classes and extremely poor performance for classes who lacks positive samples(see \ref{fig:2}). Though exchanging with server can bring lacking knowledge in some degree but facing the problem that neural weights of each model can be randomly
permuted and thus hard to fully assemble knowledge. Besides, the local model with bad performance for some class is hard to achieve promising global model by indiscriminately point-wise-averaging. In summary, the unfair competition between classes in FL clients need be effectively addressed. 

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1\columnwidth]{AAAI_figure_2.pdf}
    \end{center}
    \caption{}
    \label{fig:2}
\end{figure}

Motivated by these observations, we propose a novel algorithm that boosts the performance of standard PFL called \textbf{F}ederated \textbf{A}veraging \textbf{V}ia \textbf{B}inary \textbf{C}lassification, which adopts the “one-vs-all” framework\cite{rifkin2004defense,wen2021sphereface2} to reduce the impact among classes and be more focused on personalized
classes. Different from normal multi-class classification training, Fed# performs binary classification on training set and trains classify for each classes with shared representation(feature extractor). Concretely, given K classes in the training set, Fed# constructs K binary classification objectives where data from the target class are treated as positive samples and data from remaining classes are treated as negative samples. Employing this strategy, each classes can be more personalized and liberated from unfair competition in some degree. We then can focused on each class to personalized deal with it either imbalanced problem or lacking positive samples. Specially, we proposed a novel and effective binary loss function to address this challenge via hard-sample mining\cite{schroff2015facenet,wu2017sampling} and under-sampling \cite{yen2009cluster}, hard-sample strategy focuses on the learning of hard samples and reduces the impact of easy samples while under-sample strategy is directly abandon easy samples.

To summarize, the main contributions of this paper are:
\begin{itemize}
  \item We propose a novel FL method termed FedABC that adopts the binary classification framework. Our method can make each classes more personalized and liberated from unfair competition in heterogeneous client;
  \item We design an effective binary loss function for imbalanced problem and lacking positive samples existing among clients by utilizing hard-sample mining and under-sampling strategy;
  \item We conduct extensive experiments on two popular visual datasets(Cifar10, Mnist) under four heterogeneity settings. The results demonstrate improvements over the competitive counterparts.
\end{itemize}

%including FedAvg, FedAvg combined with balanced softmax, Fedprox, Scaffold, LG-FedAvg, FedPer, FedRep, and FedRod.

%In section~\ref{sec:Experiments}, we show experiments on multi-label datasets and results. Section~\ref{sec:Conclusion} summarizes this paper.



==> text/introduction.tex <==
\section{Introduction}
Federated learning (FL) is an emerging machine learning  paradigm that trains an algorithm across multiple decentralized clients (such as edge devices) or servers without exchanging local data samples~\cite{mcmahan2017communication}. In this big data era, large-scale data are becoming increasingly popular, but also suffer the risk of data leakage. Federated learning aims at addressing this issue by letting the clients update models using private data and the server periodically aggregate these models for multiple communication rounds. Such decentralized learning has shown its great potential to facilitate real-world applications, including healthcare~\cite{xu2021federated}, user verification~\cite{hosseini2021federated} and the Internet of Things (IoT)~\cite{zheng2022applications}.

A key challenge in federated learning is the training given non-independent and identically distributed (non-i.i.d.) data~\cite{hsieh2020non}. Due to the varied data distributions among different clients, the single global model obtained by simple averaging is hard to cater for all heterogeneous clients. Besides, clients update the global model on their local dataset, making local model misaligned and leading to weight divergence~\cite{zhao2018federated}. These issues have been found to result in unstable and slow convergence~\cite{li2020federated} and even extremely poor performance~\cite{li2021federated}.

\begin{figure}[!t]
    \begin{center}
    \includegraphics[width=1\columnwidth]{AAAI_figure_1.pdf}
    \end{center}
    \caption{An illustration of different situations of data distributions in FL: (a) ideal i.i.d; (b) long-tail; (c) and (d) lack of positive samples for some classes.}
    \label{fig:1}
\end{figure}

To deal with heterogeneity in FL, numerous solutions have been proposed, such as the ones that constrain the direction of local model update to align the local and global optimization objectives~\cite{li2020federated,karimireddy2020scaffold,acar2021federated}. Personalized federated learning (PFL)~\cite{smith2017federated} is a promising solution to addresses this challenge by jointly learning multiple personalized models, one for each client. For instance, references~\cite{collins2021exploiting,liang2020think,sun2021partialfed} exploit flexible parameter sharing strategies that only transmit partial model parameters, and the local models are regularized using a learnable global model~\cite{t2020personalized,hanzely2020lower,li2021ditto}.

However, all these approaches merely conduct an extra regularization or improve the aggregation strategy, which ignore some extraordinary situations of data distribution (see Figure~\ref{fig:1}) that often exist in FL clients. The situations can be divided into two categories: 1) imbalanced class distribution~\cite{he2009learning}, where some classes have much more/less samples than others; 2) lacking positive samples for some classes,
%only have negative samples without positive samples
and the probability of occurrence increases with the degree of heterogeneity.
%Given these facts, we further dig deeper into the process of client optimization.
%\ls{there two sequence are strange. }
In these extreme cases, if the ubiquitous Softmax function (together with cross-entropy loss)~\cite{jang2016categorical} is adopted, the normalization would enforce all the class logits summed to one, and thus induce competition among different classes. That is, increasing the confidence of one class will necessarily decrease the confidence of some other classes.
%In our case, since the imbalanced training samples and unfair competition, these two situation 
This can easily lead to over-confident predictions~\cite{guo2017calibration} for dominated classes, sub-optimal performance for minority classes and extremely poor performance for classes that lack positive samples (see Figure~\ref{fig:2}). Although communicating with the server can alleviate this issue to some extent, the neural weights of each model can be randomly permuted and thus hard to fully assemble knowledge of all clients. Besides, the classes that have poor performance in local models are hard to achieve promising global performance by indiscriminately point-wise-averaging.
%\ls{It seems that this paragraph are used to state the challenges an problem setup. This paragraph should be revised. First, we introduce the considered setting in this work, and then we explain why existing works can not perform well in this situation.}

\begin{figure}[!t]
    \begin{center}
    \includegraphics[width=1\columnwidth]{AAAI_figure_2.pdf}
    \end{center}
    \caption{An illustration of the poor performance for some classes that have few or no positive samples. The middle and last columns are results after $10$ and $50$ rounds of global aggregation and local updating, respectively.}
    \label{fig:2}
\end{figure}

To address the unfair competition between classes in FL clients,
%need to be effectively addressed. Motivated by these observations
we propose a novel method that boosts the performance of standard PFL termed \textbf{Fed}erated \textbf{A}veraging via \textbf{B}inary \textbf{C}lassification (FedABC), which adopts the well-known ``one-vs-all'' strategy~\cite{rifkin2004defense,wen2021sphereface2} to reduce the unfair competition among classes and focus more on personalized classes. Different from the traditional multi-class classification training based on Softmax, our FedABC performs binary classification for each category, where the feature extractors are shared for different classes.
%on training set and trains classify for each classes with shared representation (feature extractor).
In particular, given $K$ classes in the training set, FedABC constructs $K$ binary classification problems, where data from the target class are treated as positive samples and data from the remaining classes are treated as negative samples. By employing this strategy, the classes that have few or even no positive samples will not be suppressed by the majority categories in the prediction, and thus can be liberated from unfair competition.
%By employing this strategy, each class can be more personalized and liberated from unfair competition in some degree \ls{it is not clear how to adopt the binary classification}.
This enables us to focus on each class and personally deal with its issue of either data imbalancing or lacking of positive samples,
%\ls{rewrite this sentences}.
which is tackled by designing a novel and effective binary loss function that incorporates both the under-sampling~\cite{yen2009cluster} and hard-sample mining~\cite{schroff2015facenet,wu2017sampling} strategies. These strategies focus on the learning of hard samples and reducing the impact of easy samples. %while under-sample strategy is directly abandon easy samples. \ls{The introduced FedABC approach is not clear. We should explicitly explain the benefits of each component of FedABC.}

To summarize, the main contributions of this paper are:
\begin{itemize}
  \item We propose a novel FL method termed FedABC that adopts a binary classification strategy to increase personality of the learning for each class and liberate the different classes from unfair competition for the heterogeneous clients;
  \item We design an effective binary loss function to alleviate the imbalanced data and insufficient positive sample issues by incorporating both the hard-sample mining and under-sampling strategies.
\end{itemize}
We conduct extensive experiments on two popular visual datasets (Cifar10 and Mnist) under four heterogeneity settings. The results demonstrate the effectiveness of the proposed FedABC over the competitive baselines.

%including FedAvg, FedAvg combined with balanced softmax, Fedprox, Scaffold, LG-FedAvg, FedPer, FedRep, and FedRod.

%In section~\ref{sec:Experiments}, we show experiments on multi-label datasets and results. Section~\ref{sec:Conclusion} summarizes this paper.



==> text/methodology-V1.tex <==
\section{Federated Averaging Via Binary Classification}
\label{sec:Method_Fed\#}
\begin{figure*}[t]   
    \begin{center}      
    \includegraphics[width=2\columnwidth, height=0.5\textwidth]{Overview-V2.pdf}
    \end{center}
    \caption{\textbf{Overview of the proposed federated averaging via binary classification (FedABC) method}. Our framework is based on the vanilla federated learning paradigm where the server orchestrates the learning amongst clients and is responsible for aggregating the client personalized model parameters. In the local training process, FedABC adopts the “one-vs-all” training strategy that learns an independent classifier for each class while the feature extractor is shared. The data from the target class are treated as positive samples and the remaining data are treated as negative samples. Due to Non-iid dataset, some classes face the imbalanced problem while some classes have no positive samples.}
    \label{pipeline}
\end{figure*}

In this section, we present the proposed personalized FedABC, our method bases on vanilla FedAvg framework and utilize the personalized model to complete personalization. A central server orchestrates the learning
amongst clients and is responsible for parameter aggregation after receiving locally trained models on the edge as
depicted in \ref{pipeline} left part. The critical innovation in our work consists of two parts: the proposed FL imbalanced binary loss function and the binary classification training framework.



\subsection{FL binary loss function}
The goal of our method is to train the efficient binary classification for each classes, a naive binary loss formulation of class $c$ from the cross entropy (CE) loss is given by following:

\begin{equation}
    L_{\textit{BCE}}(c,p,y)=-[y{\log}(p)+(1-y){\log}(1-p)]
\label{BCE}
\end{equation}

where probability $p:=\sigma({g}(x;\theta^{p};\theta^{h}), p\in[0,1]$ is the output after the operation of sigmoid activation, and $y = 0||1$ is the samples true label. According to the class situation mentioned above, we rewrite the naive binary loss function \ref{BCE} to the following formulation:
\begin{equation}
L_{\textit{BCE}}(c,p,y)=\left\{
\begin{aligned}
&-[y{\log}(p)+(1-y){\log}(1-p)], & c \in C^{p} \\
&-{\log}(1-p), & c \in C^{n}\\
\end{aligned}
\right.
\end{equation}

Regard to the $C^{P}$ facing the imbalance problem, no modification is done and same as the \ref{BCE} while we neglect the positive part of loss for the $C^{n}$ since its lacking positive samples. Employing this binary classification training framework, the unfair competition can be liberated but the imbalance problem within binary classification may be more serious, since there are a great many negative samples and few positive samples, especially in huge heterogeneous setting. To address this challenging problem, we adopt under-sampling and the hard sample mining strategy to alleviate it.

\subsubsection{Incorporating Under-sampling}

The under-sampling strategy aimed to abandon low value samples for the majority classes and alleviate the imbalanced problem through modifying the number of training samples. To quantity the value of samples, we utilize the probability $p$ as the metric, the model will add samples whose value is larger than the setting margin into the current training batch, and the remaining will be abandoned. The formulation of binary loss function integrating under-sampling strategy is defined as the following:

\begin{equation}
\begin{split}
L_{\textit{BCE}}^{p}(p,y)&=\left\{
\begin{aligned}
&-{\log}(p), & y=1, p<m^{p} \\
&-{\log}(1-p), & y=0, p>m^{n}\\
\end{aligned}
\right.\\
L_{\textit{BCE}}^{n}(p,y)&=-{\log}(1-p), \quad \quad \quad \quad\quad y=0, p>m^{nn}
\end{split}
\label{BCE_under_sampling}
\end{equation}

The formulation for $C^{p}$ is denoted as $L_{\textit{BCE}}^{p}(c,p,y)$, while $L_{\textit{BCE}}^{n}(c,p,y)$ is denoted for $C^{n}$ who only have negative samples. Some positive samples have already get nice probability near one, so that the positive samples with low probability are valuable for the model training, and need to be better trained. Instead, we maintain the samples whose $p$ is large with respect for negative samples. Three hyper parameter $m^{p},m^{n},m^{nn}$ in different clients can be various but we make them equal in the simplest way.

\subsubsection{Incorporating Hard Sample Mining}
Another crucial technique for a good loss function is the strategy for mining
hard samples. The classic Focal Loss\cite{lin2017focal} is widely-used to alleviate the imbalance problem, it utilities hard sample mining strategy to rebalance the loss contribution of easy samples and hard samples. In our method, we also follow this promising art to alleviate the imbalance problem by focusing more on hard samples and lower the importance of easy samples, the formulation of our final loss function can be given as the following:
\begin{equation}
\begin{split}
L_{\textit{BCE}}^{p}(p,y)&=\left\{
\begin{aligned}
&-(1-p)^{\alpha}{\log}(p), & y=1, p<m^{p} \\
&-p^{\alpha}{\log}(1-p), & y=0, p>m^{n}\\
\end{aligned}
\right.\\
L_{\textit{BCE}}^{n}(p,y)&=-p^{\alpha}{\log}(1-p), \quad \quad \quad y=0, p>m^{nn}\!\!\!
\end{split}
\label{BCE_final}
\end{equation}
where $\alpha$ is the hyper parameter to control the degree of hard sample mining.


\begin{small}
\begin{algorithm}[!t]
	\caption{Federated Averaging via Binary classification}
	\label{alg} 
	\begin{algorithmic}
		\STATE \textbf{Input:} $m$ clients, $\mathcal{S}^{i}$ at the $i$-th client.
		\STATE Server initializes parameters $\theta^{0}$.
		\STATE Server sends the initialization to clients.
	    \STATE \textbf{for} t=0,1,2,...,T-1 \textbf{do}:
	    \STATE \quad Server sends $\theta^{t}$ to the $i$-th client
	    \STATE \quad \textbf{for} i=1,2,...,C \textbf{do}
	    \STATE \quad \quad $\theta^{t}_{i} \leftarrow\theta^{t}_{i}, -\eta \nabla_{\theta^{t}} \hat{\mathcal{R}}\left(\mathcal{S}^{i},\theta_{i}\right)$
	    \STATE \quad \quad $\text{where } \hat{\mathcal{R}}\left(\mathcal{S}^{i},\theta_{i}\right)=\mathbb{E}\left[\mathcal{L}_{(\boldsymbol{x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\theta_{i} \right)\right]$

	    
	    \STATE \quad \quad
	    The $i$-th client maintain $\theta_{i}^{t}$ as current PM.
	    \STATE \quad \quad 
	    The $i$-th client sends $\theta^{t}_{i}$ to the server.
	    \STATE \quad \textbf{end for}
	    \STATE \quad Server updates the model parameters by averaging :\\
	    \quad $\theta ^{t+1}=\frac{1}{C} \sum\limits_{i\in [C] }\theta^{t}_{i}$
	    \STATE \textbf{end for}
	    \STATE \textbf{Output:} PM$:\{\sum_{i}^{m}\theta_{i}^{\mathrm{T}}\}$,  GM$:\{\theta^{\mathrm{T}}\}$
	\end{algorithmic} 
\end{algorithm}
\end{small}


\subsection{Binary classification training framework}

Our method adopts the binary class training framework with FL. Specially, a encoder maps the input data into the low-dimensional feature, the \textbf{sigmoid} activation is applied and then get the final logit, the logit lies in the interval $[0,1]$. Our method trains a classify for each classes to complete binary classification task under the shared feature extractor, the pipeline is depicted in \ref{pipeline} right part. In practice, the classify is the fully connected layer same as the normal training paradigm and just output one-dimensional individual logit. Our method do not need any extra modifications on the structure of neural network or others, and just need apply sigmoid activation and then utilize our binary loss function\ref{BCE_final}.

The empirical loss of the $i$-th client on the local dataset $\mathcal{S}^{i}$ can be given by:
\begin{align}
\mathbb{E}\left[\mathcal{L}_{(\boldsymbol{x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\theta_{i} \right)\right]:=&\frac{1}{|\mathcal{S}^{i}|}\sum_{j}^{C_{i}^{p}}{L}^{p}_\textit{BCE}(\mathcal{S}^{i};\theta_{i}) \nonumber\\
&+
\frac{1}{|\mathcal{S}^{i}|}\sum_{j}^{C_{i}^{n}} L_{\textit{BCE}}^{n}(\mathcal{S}^{i};\theta_{i})
\end{align}
Since our binary loss function have different forms in term with $C_{i}^{p}$ and $C_{i}^{p}$, so that we do not merge them into one. Employing this training strategy can liberate unfair competition between classes in the classify and be more focused on personalized classes. In our method, each classes treat the training data as positive samples or negative samples. Though also existing imbalanced and lacking positive samples problem, but we can adopt customized binary loss function\ref{BCE_final} to alleviate it. In Algorithm~\ref{alg}, we summarize the learning procedure of our FedABC method.



==> text/methodology.tex <==
\section{Federated Averaging Via Binary Classification}

\begin{figure*}[t]   
    \begin{center}      
    \includegraphics[width=2\columnwidth, height=0.5\textwidth]{Overview-V2.pdf}
    \end{center}
    \caption{\textbf{Overview of the proposed federated averaging via binary classification (FedABC) framework}, which is based on the vanilla federated learning paradigm, where the server orchestrates the learning amongst clients and is responsible for aggregating the client personalized model parameters. In the local training process, FedABC adopts the ``one-vs-all'' training strategy that learns an independent binary classifier for each category, while the feature extractor is shared. This may lead to severe class imbalancing problem, and some classes may have no positive samples, and therefore a novel personalized binary classification loss is designed.}
    \label{pipeline}
\end{figure*}
%The data from the target class are treated as positive samples and the remaining data are treated as negative samples.

In this section, we present the proposed FedABC, our method is based on the vanilla federated by averaging framework, where a central server exchange averaging model parameter with clients as
depicted in \ref{pipeline} left part. In the client training process, different from the normal training method adopting softmax, FedABC adopts the ``one-vs-all'' training strategy as
depicted in \ref{pipeline} right part. The critical innovation in our method consists of two components: the binary loss function and the binary classification training framework.

\subsection{FL binary loss function}
The goal of our method is to train a efficient binary classifier for each class, a naive binary loss formulation of class $c$ from the cross entropy (CE) loss is given by following:

\begin{equation}
    L_{\textit{BCE}}(c,q,y)=-[y{\log}(q)+(1-y){\log}(1-q)]
\label{BCE}
\end{equation}

where probability $q:=\sigma({g}(x;\boldsymbol{\theta}^{f};\boldsymbol{\theta}^{h}), q\in[0,1]$ is the output after the operation of sigmoid activation, and $y = 0, 1$ is the samples true label. According to the class situation mentioned above, we rewrite the binary loss function (\ref{BCE}) into the following formulation:
\begin{equation}
L_{\textit{BCE}}(c,q,y)=\left\{
\begin{aligned}
&-[y{\log}(q)+(1-y){\log}(1-q)], & c \in C^{q} \\
&-{\log}(1-q), & c \in C^{n}\\
\end{aligned}
\right.
\label{FL_BCE}
\end{equation}

Regards the $C^{p}$ facing the imbalance problem, no extra modification is operated and same as the (\ref{BCE}), while we neglect the positive part loss item of the $C^{n}$ due to its lacking positive samples. By employing this binary training framework, classes can avoid the forced and competitive normalization from softmax, and thus the unfair competition can be liberated to a certain extent. However, the imbalance problem within binary classification may be serious because of existing many negative samples and few positive samples for the corresponding class in most cases. To address this challenging problem, we adopt under-sampling and the hard sample mining strategy to alleviate it.

\paragraph{Incorporating Under-sampling.} 
The under-sampling strategy aimed to abandon low-value samples and re-balance data distribution to alleviate the imbalanced problem. To quantity the value of samples, we utilize the probability $p$ as the importance metric, the model will add samples whose importance value is larger than the setting margin into the current training batch, and the remaining will be abandoned directly. This process is dynamic for each training epoch. The formulation of binary loss function incorporating the under-sampling strategy is defined as the following:
\begin{equation}
\begin{split}
L_{\textit{BCE}}^{p}(q,y)&=\left\{
\begin{aligned}
&-{\log}(q), & y=1, q<m^{p} \\
&-{\log}(1-q), & y=0, q>m^{n}\\
\end{aligned}
\right.\\
L_{\textit{BCE}}^{n}(q,y)&=-{\log}(1-q), \quad \quad  y=0, q>m^{nn}
\end{split}
\label{BCE_under_sampling}
\end{equation}

The binary loss function for $C^{p}$ is denoted as $L_{\textit{BCE}}^{p}(c,p,y)$, while $L_{\textit{BCE}}^{n}(c,p,y)$ is denoted for $C^{n}$ who only have negative samples. Some positive samples have already achieved a nice probability near one, therefore the positive samples with low probability are valuable for the model training and need to be better trained in this epoch. Instead, we maintain the negative samples whose $p$ is large than the margin. Three hyperparameters $m^{p},m^{n},m^{nn}$ is the setting margin for the corresponding class. In practice, these three parameters in different clients can be various but we make them equal in the simplest way.

\paragraph{Incorporating Hard Sample Mining.}
Another crucial technique for a better loss function is the strategy for mining
hard samples. The famous Focal Loss\cite{lin2017focal} is widely-used to alleviate the imbalance problem and achieve expected performance, it utilizes the hard sample mining strategy to re-balance the loss contribution of easy samples and hard samples. In our method, we also follow this hard sample mining method to alleviate the imbalance problem by focusing more on hard samples and lowering the significance of easy samples, the formulation of our final binary loss function can be given as the following:
\begin{equation}
\begin{split}
L_{\textit{BCE}}^{p}(q,y)&=\left\{
\begin{aligned}
&-(1-q)^{\alpha}{\log}(q), & y=1, q<m^{p} \\
&-q^{\alpha}{\log}(1-q), & y=0, q>m^{n}\\
\end{aligned}
\right.\\
L_{\textit{BCE}}^{n}(q,y)&=-q^{\alpha}{\log}(1-q), \quad \quad \quad y=0, q>m^{nn}\!\!\!
\end{split}
\label{BCE_final}
\end{equation}
where $\alpha$ is the hyper parameter to control the degree of hard sample mining.

\begin{small}
\begin{algorithm}[!t]
	\caption{Federated Averaging via Binary classification}
	\label{alg} 
	\begin{algorithmic}
		\STATE \textbf{Input:} $m$ clients, $\mathcal{S}^{i}$ at the $i$-th client.
		\STATE Server initializes parameters $\boldsymbol{\theta}^{0}$.
		\STATE Server sends the initialization to clients.
	    \STATE \textbf{for} t=0,1,2,...,T-1 \textbf{do}:
	    \STATE \quad Server sends $\theta^{t}$ to the $i$-th client
	    \STATE \quad \textbf{for} i=1,2,...,C \textbf{do}
	    \STATE \quad \quad $\theta^{t}_{i} \leftarrow\boldsymbol{\theta^{t}}_{i}, -\eta \nabla_{\boldsymbol{\theta^{t}}} \hat{\mathcal{R}}\left(\mathcal{S}^{i},\boldsymbol{\theta}_{i}\right)$
	    \STATE \quad \quad $\text{where } \hat{\mathcal{R}}\left(\mathcal{S}^{i},\boldsymbol{\theta}_{i}\right)=\mathbb{E}\left[\mathcal{L}^{\textit{BCE}}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right]$

	    
	    \STATE \quad \quad
	    The $i$-th client maintain $\boldsymbol{\theta}_{i}^{t}$ as current PM.
	    \STATE \quad \quad 
	    The $i$-th client sends $\boldsymbol{\theta}^{t}_{i}$ to the server.
	    \STATE \quad \textbf{end for}
	    \STATE \quad Server updates the model parameters by averaging :\\
	    \quad $\boldsymbol{\theta} ^{t+1}=\sum\limits_{i\in [C] } \frac{|\mathcal{S}^{i}|}{|\mathcal{S}|} \boldsymbol{\theta}^{t}_{i}$
	    \STATE \textbf{end for}
	    \STATE \textbf{Output:} PM$:\{\sum_{i}^{m}\boldsymbol{\theta_{i}}^{\mathrm{T}}\}$,  GM$:\{\boldsymbol{\theta}^{\mathrm{T}}\}$
	\end{algorithmic} 
\end{algorithm}
\end{small}


\subsection{Binary classification training framework}

Our method adopts the binary training strategy in the local learning process. Specially, an encoder including an embedding network and a classifier first maps the input data into the low-dimensional feature, the \textbf{sigmoid} activation is applied to it and then we get the final logit, the resulted logit lies in the interval $[0,1]$. Our method trains an independent classifier for each class to complete the binary classification task and the feature extractor is shared, more details are depicted in \ref{pipeline}. In practice, the classifier is the normal fully connected layer, and just outputs one-dimensional individual logit for the corresponding class. Our method does not need any extra modifications on the structure of the neural network or others, and only need to apply sigmoid activation and adopt our proposed binary loss function(\ref{BCE_final}).

The empirical loss of the $i$-th client on the local dataset $\mathcal{S}^{i}$ can be given by:
\begin{equation}
\begin{split}
\mathbb{E}\left[\mathcal{L}^{\textit{BCE}}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta_{i}} \right)\right]:=&\frac{1}{|\mathcal{S}^{i}|} \left(\sum_{j}^{C_{i}^{p}}{L}^{p}_\textit{BCE}(\mathcal{S}^{i};\boldsymbol{\theta}_{i})\right.\\
&\left.+\sum_{j}^{C_{i}^{n}} L_{\textit{BCE}}^{n}(\mathcal{S}^{i};\boldsymbol{\theta}_{i}) \right).
\end{split}
\end{equation}
Since our binary loss function have different forms in term with $C_{i}^{p}$ and $C_{i}^{p}$, we do not merge them together. Employing this training strategy can liberate unfair competition between classes in the classifier and be more focused on personalized classes. In our method, each class treats the training data as positive samples or negative samples. Though also existing imbalanced and lacking positive samples problem, we can adopt the customized binary loss function mentioned above (\ref{BCE_final}) to alleviate it. In Algorithm~\ref{alg}, we summarize the learning procedure of our proposed FedABC method.



==> text/problem_setup-V1.tex <==
\section{Problem Formulation}
\label{sec:Problem_Formulation}
\subsection{Personalized Federated Learning.}
In this work, we consider a typical PFL setting for supervised learning, i.e., the multi-class classification. We suppose that there are $m$ clients and $C$ classes in total. For $i \in [m]$, $i$-th client has individual data distribution $\mathcal{D}_{i}$, where some classes have much more samples and the remaining classes have less, these classes who have positive samples are denoted as $C_{i}^{p}$. Meanwhile some classes have no positive samples and only have negative samples, which are denoted as $C_{i}^{n}$. %
%
The ${i}$-th client has access to the local dataset $\mathcal{S}^{i}=\{(\mathbf{x}_{i}^{1},y_{i}^{1}),(\mathbf{x}_{i}^{2},y_{i}^{2}),\cdots,(\mathbf{x}^{n_{i}}_{i},y_{i}^{n_{i}})\} $. %
%
A neural network $\theta_{i}$ of the $i$-th client splits as two parts: an embedding network $f: \chi \rightarrow \mathbb{Z}$ parameterized by $\theta^{p}_{i} $ maps the input $\mathbf{x}$ to the latent feature, i.e., $\mathbb{Z}:= f(\mathbf{x};\theta_{i}^{p})$, and a predictor $h:\mathbb{Z} \rightarrow \mathbf{y}$ parameterized by $\theta^{h}_{i}$ maps latent feature to the logits $\mathbf{y}$ , i.e.,  $y:=h(f(x;\theta_{i}^{p});\theta_{i}^{h})$. 
The corresponding feature extractor part and predictor part of the global model $\theta$ achieved by averaging are defined as $\theta^{p}$ and $\theta^{h}$, respectively. The non-linear activation applied to $y$ and is defined as $\sigma(\cdot)$, so that the output of the neural network can be defined as $\sigma(h(f(x;\theta^{p});\theta^{h}))$. we short it as $p:=\sigma({g}(x;\theta^{p};\theta^{h}))$. %
%
Due to our method employs the binary classification framework, the activation applied in our work is $\textbf{sigmoid}$, which maps the input into the $[0,1]$. For $i\in[m],j\in[C]$, the binary loss for the corresponding class can be defined as $\ell_{i}^{j}(x_{i},y_{i};\theta)$. We formulate PFL problem according to \cite{hanzely2021personalized} into the following optimization problem:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{(\boldsymbol{x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right].
\end{gathered}
\label{general-PFL}
\end{equation}
PFL learns a model $\theta_{i}$ for each client $m$, whose goal is to perform well on the local dataset $\mathcal{S}_{i}$ and the local model parameters $\theta_{i}$ are often initialized with the global model $\theta$. Many existing works add a regularizer either on the server-side to improve the aggregation scheme or on the client-side to improve the local optimization, but there is no agreed objective function so far. Most existing FL works exploiting to achieve a better global model can be easily adopted in PFL without extra processing steps. This is achieved by utilizing the locally trained model as a personalized model. To  formulate the PFL problem more comprehensively, we formulate this problem into three categories: 1) Adding a regularizer on the server side; 2) Adding a regularizer on the client side; 3) Adding regularizers on both the client side and the server side; Firstly, we formulate the PFL problem that adding a regularizer on the server-side into the following optimization task:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right) \\
\qquad\qquad\qquad\qquad\qquad +\mathcal{R}(\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m},\boldsymbol{\Omega}), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{(\boldsymbol{x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right],\\
\end{gathered}
\label{Server-PFL}
\end{equation}
where $\mathcal{R}$ is the regularizer and $\boldsymbol{\Omega}$ is the useful information including the averaging model parameters, gradients, feature distribution, or the model fusion strategy, etc. The extra processing step is done on the global model to improve the assembly of knowledge, and thus clients can receive better global initialization and further improve PFL accuracy. Besides, adding a regularizer on the client-side is encouraged to achieve better generalization and directly improve the personalized model performance. We also formulate this PFL problem that adding a regularizer on the client-side into the following optimization task:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{(\boldsymbol{x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right]+\mathcal{R}(\boldsymbol{\theta}_{i},\boldsymbol{\theta},\boldsymbol{\Omega}).
\end{gathered}
\label{Client-PFL}
\end{equation}
In the end, adding a regularized on bath side can be simultaneously done, and the formulation of this problem can be simply achieved by combining (\ref{Server-PFL}) and (\ref{Client-PFL}). In our work, we propose a novel method that adopts binary training strategy to tackle the imbalanced problem and boost the generalization of client model. This method doesn't need any extra information or other proxy data. The objective of our work can be easily formulated by (\ref{general-PFL}).


\subsection{Differences between generic FL and PFL.}
PFL trains a local model for each clients and generic FL only holding a global model. We follow the concept proposed in ~\cite{chen2021bridging} that claimed that PFL also has the global model and the generic FL also have the personalized model, and thus the generic FL and PFL can be easily converted to each other. Regarding PFL, the global model is the averaging model on the server-side. Meanwhile, the generic FL also has the locally trained model on the client side and can be treated as the client personalized model undoubtedly. So that the critical difference between these two learning paradigms is \textbf{which model is tested}. If the global model is tested on the IID test set, so the resulted accuracy is the performance of generic FL, while the personalized models are tested on the local Non-iid test set, the averaging accuracy of each local model will be the performance of PFL.



==> text/problem_setup.tex <==
\section{Problem Formulation}
\label{sec:Problem_Formulation}
\subsection{Personalized Federated Learning}
In this work, we consider a typical PFL setting for supervised learning, i.e., the multi-class classification. We suppose that there are $m$ clients and $C$ classes in total. For $i \in [m]$, the $i$-th client has individual data distribution $\mathcal{D}_{i}$, where some classes have many samples and the remaining classes have much fewer. The classes that have positive samples are denoted as $C_{i}^{p}$, and some classes that have no positive samples are denoted as $C_{i}^{n}$. %
%
The ${i}$-th client has access to the local dataset $\mathcal{S}^{i}=\{({x}_{i}^{1},y_{i}^{1}),({x}_{i}^{2},y_{i}^{2}),\cdots,({x}^{n_{i}}_{i},y_{i}^{n_{i}})\} $. %
%
The neural network parameter $\boldsymbol{\theta}_{i}$ of the $i$-th client consists of two parts: an embedding network $f: \mathcal{X} \rightarrow \mathcal{Z}$ parameterized by $\boldsymbol{\theta}^{f}_{i} $ maps the input ${x}$ to the latent feature, i.e., ${z}:= f({x};\boldsymbol{\theta}_{i}^{f})$, and a predictor $h:\mathcal{Z} \rightarrow \mathcal{Y}$ parameterized by $\boldsymbol{\theta}^{h}_{i}$ maps latent feature to the logits ${y}$ , i.e.,  $y:=h(f({x}; \boldsymbol{\theta}_{i}^{f}); \boldsymbol{\theta}_{i}^{h})$.
The corresponding feature extractor part and predictor part of the global model $\theta$ achieved by averaging are defined as $\boldsymbol{\theta}^{f}$ and $\boldsymbol{\theta}^{h}$, respectively. A non-linear activation $\sigma(\cdot)$ is applied to $y$, so the output of the neural network can be defined as $\sigma(h(f({x}; \boldsymbol{\theta}^{f}), \boldsymbol{\theta}^{h}))$, and we rewrite it as $q:=\sigma({g}({x};\boldsymbol{\theta}^{f};\boldsymbol{\theta}^{h}))$. %
%
Due to our method employs the binary classification framework, the activation applied in our work is $\textbf{sigmoid}$, which maps the input into the $[0,1]$. For $i\in[m],j\in[C]$, the binary loss for the corresponding class can be defined as $\ell_{i}^{j}(x_{i},y_{i};\boldsymbol{\theta})$. We formulate PFL problem according to \cite{hanzely2021personalized} into the following optimization problem:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right].
\end{gathered}
\label{general-PFL}
\end{equation}
PFL learns a model $\boldsymbol{\theta_{i}}$ for each client $m$, whose goal is to perform well on the local dataset $\mathcal{S}_{i}$, and the local model parameters $\boldsymbol{\theta_{i}}$ are often initialized with the global model $\boldsymbol{\theta}$. In PFL, many existing works add a regularizer either on the server-side to improve the aggregation scheme or on the client-side to improve the local optimization, but there is no agreed objective function so far. Most existing generic FL works exploiting to achieve a better global model can be easily adopted in PFL without extra processing steps. This is achieved by utilizing the locally trained model as its personalized model. To formulate the PFL problem more comprehensively, we formulate this problem into three categories: 1) Adding a regularizer on the server side; 2) Adding a regularizer on the client side; 3) Adding regularizers on both the client side and the server side; Firstly, we formulate the PFL problem that adding a regularizer on the server-side into the following optimization task:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right) \\
\qquad\qquad\qquad\qquad\qquad +\mathcal{R}(\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m},\boldsymbol{\Omega}), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right],\\
\end{gathered}
\label{Server-PFL}
\end{equation}
where $\mathcal{R}$ is the regularizer and $\boldsymbol{\Omega}$ is the useful information including the averaging model parameters, gradients, feature distribution, or the model fusion strategy, etc. The extra processing step is done on the global model to improve the assembly of knowledge, and thus clients can receive better global initialization and further improve PFL accuracy. Besides, adding a regularizer on the client-side is encouraged to achieve better generalization and directly improve the personalized model performance. We also formulate this PFL problem that adding a regularizer on the client-side into the following optimization task:
\begin{equation}
\begin{gathered}
\small
\min _{\left\{\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right\}} f\left(\boldsymbol{\theta},\boldsymbol{\theta}_{1}, \cdots, \boldsymbol{\theta}_{m}\right)=\frac{1}{m} \sum_{i=1}^{m}F_{i}\left(\boldsymbol{\theta}_{i}\right), \\
F_{i}\left(\boldsymbol{\theta}_{i}\right):=\mathbb{E}\left[\mathcal{L}_{({x}, y) \sim \mathcal{D}_{i}}\left(\mathcal{S}^{i};\boldsymbol{\theta}_{i} \right)\right]+\mathcal{R}(\boldsymbol{\theta}_{i},\boldsymbol{\theta},\boldsymbol{\Omega}).
\end{gathered}
\label{Client-PFL}
\end{equation}
In the end, adding a regularized on bath side can be simultaneously done, and the formulation of this problem can be simply achieved by combining (\ref{Server-PFL}) and (\ref{Client-PFL}). In our work, we propose a novel method that adopts binary training strategy to tackle the imbalanced problem and boost the generalization of client model. This method doesn't need any extra information or other proxy data. The objective of our work can be easily formulated by (\ref{general-PFL}).


\subsection{Differences between generic FL and PFL}
PFL trains a local model for each clients and generic FL only holding a global model. We follow the concept proposed in ~\cite{chen2021bridging} that claimed that PFL also has the global model and the generic FL also have the personalized model, and thus the generic FL and PFL can be easily converted to each other. Regarding PFL, the global model is the averaging model on the server-side. Meanwhile, the generic FL also has the locally trained model on the client side and can be treated as the client personalized model undoubtedly. So that the critical difference between these two learning paradigms is \textbf{which model is tested}. If the global model is tested on the IID test set, so the resulted accuracy is the performance of generic FL, while the personalized models are tested on the local Non-iid test set, the averaging accuracy of each local model will be the performance of PFL.


